AbacusSummit: A Massive Set of High-Accuracy, High-Resolution $N$-Body Simulations

We present the public data release of the AbacusSummit cosmological $N$-body simulation suite, produced with the $\texttt{Abacus}$ $N$-body code on the Summit supercomputer of the Oak Ridge Leadership Computing Facility. $\texttt{Abacus}$ achieves $\mathcal{O}\left(10^{-5}\right)$ median fractional force error at superlative speeds, calculating 70M particle updates per second per node at early times, and 45M particle updates per second per node at late times. The simulation suite totals roughly 60 trillion particles, the core of which is a set of 139 simulations with particle mass $2\times10^{9}\,h^{-1}\mathrm{M}_\odot$ in box size $2\,h^{-1}\mathrm{Gpc}$. The suite spans 97 cosmological models, including Planck 2018, previous flagship simulation cosmologies, and a linear derivative and cosmic emulator grid. A sub-suite of 1883 boxes of size $500\,h^{-1}\mathrm{Mpc}$ is available for covariance estimation. AbacusSummit data products span 33 epochs from $z=8$ to $0.1$ and include lightcones, full particle snapshots, halo catalogs, and particle subsets sampled consistently across redshift. AbacusSummit is the largest high-accuracy cosmological $N$-body data set produced to date.

==> cosmo_test_table.tex <==
\begin{landscape}
\begin{longtable}{ | p{5cm} | *{15}{c|} }
\hline\endhead  % header material
\hline\endfoot  % footer material
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
\end{longtable}
\end{landscape}

==> cosmology_table.tex <==
\begin{landscape}

\label{tab:cosmo}
% \small
\setlength\tabcolsep{3pt}
  \begin{longtable}{>{\raggedright\arraybackslash}c%
   >{\raggedright\arraybackslash}p{5.5cm}%
   >{\centering\arraybackslash}c%
   >{\centering\arraybackslash}c%
   >{\centering\arraybackslash}c%
   >{\centering\arraybackslash}c%
   >{\centering\arraybackslash}c%
   >{\centering\arraybackslash}c%
   >{\centering\arraybackslash}c%
   >{\centering\arraybackslash}c%
   >{\centering\arraybackslash}N{2cm}%
   >{\centering\arraybackslash}c%
   >{\centering\arraybackslash}c%
   >{\centering\arraybackslash}c%
   >{\centering\arraybackslash}c%
  }
  
  
%   { p{1cm} p{6cm} ccccccccccccc }
    Name & Description & $\omega_b$ & $\omega_{c}$ & $h$ & $10^9 A_s$ & $n_s$ & $\alpha_s$ & \code{N\_ur} & \code{N\_ncdm} &	\code{omega\_ncdm} (e-4)&	\code{w0\_fld} &	\code{wa\_fld} &	$\sigma_{8,m}$ &	$\sigma_{8,cb}$ \\
    \midrule

\code{cosm000}    & Baseline $\Lambda$CDM, Planck 2018 \code{base\_plikHM\_TTTEEE\_lowl\_lowE\_lensing} mean & 0.02237 &  0.1200   & 0.6736 & 2.0830   & 0.9649 & 0.0      &   2.0328 & 1      &  6.4420 & -1.0   & 0.0    & 0.807952 & 0.811355                          \\
\code{cosm001}    & WMAP9+ACT+SPT $\Lambda$CDM, Calabrese++ 2017                                 & 0.02242 &  0.1134   & 0.7030 & 2.0376   & 0.9638 & 0.0      &   2.0328 & 1      &  6.4420 & -1.0   & 0.0    & 0.776779 & 0.780222  \\
\code{cosm002}    & wCDM with thawing model $w_0$ = -0.7, $w_a$ = -0.5                         & 0.02237 &  0.1200   & 0.6278 & 2.3140  & 0.9649 & 0.0      &   2.0328 & 1      &  6.4420 & -0.7   & -0.5    & 0.808189 & 0.811577  \\
\code{cosm003}    & $N_{\textrm{eff}}$=3.70, from \code{base\_nnu\_plikHM\_TT\_lowl\_lowE\_Riess18\_post\_BAO}        & 0.02260 &  0.1291   & 0.7160 & 2.2438   & 0.9876 & 0.0      &   2.6868 & 1      &  6.4420 & -1.0   & 0.0    & 0.855190 & 0.858583  \\
\code{cosm004}    & Low $\sigma_{8,m}$ = 0.75, otherwise Baseline $\Lambda$CDM                   & 0.02237 &  0.1200   & 0.6736 & 1.7949   & 0.9649 & 0.0      &   2.0328 & 1      &  6.4420 & -1.0   & 0.0    & 0.749999 & 0.753159  \\
\code{cosm009}    & Baseline $\Lambda$CDM with massless neutrinos matching $\Omega_{cb}$ \& $\sigma_{8,cb}$  & 0.02237 &  0.1200   & 0.6736 & 2.0417   & 0.9649 & 0.0      &   3.046  & 0      & 0.0        & -1.0   & 0.0    & 0.811362 &0.811362  \\
\code{cosm010}    & AbacusCosmos Planck $\Lambda$CDM cosmology                                   & 0.02222 &  0.1199   & 0.6726 & 2.100    & 0.9652 & 0.0      &   3.04   & 0      & 0.0        & -1.0   & 0.0    & 0.823630 &0.823630  \\
  \code{cosm012}    & Euclid Flagship1 $\Lambda$CDM, $\sigma_{8,m}$=0.8279                               & 0.02200 &  0.1212   & 0.6700 & 2.1000   & 0.9600 & 0.0      &   3.046  & 0      & 0.0        & -1.0   & 0.0    & 0.827899 &0.827899  \\
\code{cosm013}    & Euclid Flagship2 $\Lambda$CDM, $\sigma_{8,m}$=0.813715, $\sigma_{8,cb}$=0.817135         & 0.02200 &  0.1206   & 0.6700 & 2.1000   & 0.9600 & 0.0      &   2.0328 & 1      &  6.4420 & -1.0   & 0.0    & 0.813715 & 0.817135  \\
\code{cosm014}    & OuterRim $\Lambda$CDM, $\sigma_8$  =0.80                                           & 0.02258 &  0.1109   & 0.7100 & 2.1591   & 0.9630 & 0.0      &   3.046  & 0      & 0.0        & -1.0   & 0.0    & 0.800000 &0.800000  \\
\code{cosm015}    & DarkSky $\Lambda$CDM, $\sigma_8$  =0.835                                           & 0.02215 &  0.1175   & 0.6880 & 2.1852   & 0.9688 & 0.0      &   3.046  & 0      & 0.0        & -1.0   & 0.0    & 0.835005 &0.835005  \\
\code{cosm016}    & Horizon Run 4 $\Lambda$CDM, $\sigma_8$  =0.7937                                    & 0.02281 &  0.1120   & 0.7200 & 2.0996   & 0.9600 & 0.0      &   3.046  & 0      & 0.0        & -1.0   & 0.0    & 0.793693 &0.793693  \\
\code{cosm017}    & IllustrisTNG $\Lambda$CDM, $\sigma_8$  =0.8159                                     & 0.02230 &  0.1194   & 0.6774 & 2.0671   & 0.9667 & 0.0      &   3.046  & 0      & 0.0        & -1.0   & 0.0    & 0.815903 &0.815903  \\
\code{cosm018}    & MultiDark Planck $\Lambda$CDM, $\sigma_8$  =0.8228                                 & 0.02214 &  0.1189   & 0.6777 & 2.1022   & 0.9600 & 0.0      &   3.046  & 0      & 0.0        & -1.0   & 0.0    & 0.819708 &0.819708 \\
\code{cosm019}    & Baseline $\Lambda$CDM with two 0.06 eV neutrinos                             & 0.02237 &  0.1200   & 0.6683 & 2.1353  & 0.9649 & 0.0      &   1.0196 & 2      &  6.4420 each & -1.0   & 0.0    &0.805050 & 0.811826  \\
\code{cosm020}    & Baseline $\Lambda$CDM with three 0.06 eV neutrinos                           & 0.02237 &  0.1200   & 0.6623 & 2.1867  & 0.9649 & 0.0      &   0.0000 & 3      &  6.4420 each & -1.0   & 0.0    & 0.801960 & 0.812073  \\
\code{cosm021}   & MassiveNUs massless base                                                     & 0.02254 &  0.12446  & 0.700  &, 2.1000 & 0.9700 & 0.0     & 3.046  & 0      & 0.0        & -1.0   & 0.0    & 0.849842 & 0.849842 \\ 
\code{cosm022}   & MassiveNUs with one 0.1 eV massive neutrino species & 0.02254 &  0.12339  & 0.700  & 2.1000 & 0.9700 & 0.0     & 2.0328 & 1      & 0.001074   & -1.0   & 0.0    & 0.824961 & 0.830296  \\
\code{cosm100}    & Baseline +2\% $ln(\omega_b)$                                             & 0.02282 &  0.1200   & 0.6777 & 2.0934  & 0.9649 & 0.0      &   2.0328 & 1      &  6.4420 & -1.0   & 0.0    & 0.808181 & 0.811575  \\
\code{cosm101}    & Baseline -2\% $ln(\omega_b)$                                              & 0.02193 &  0.1200   & 0.6696 & 2.0751  & 0.9649 & 0.0      &   2.0328 & 1      &  6.4420 & -1.0   & 0.0    & 0.808156 & 0.811570  \\
\code{cosm102}    & Baseline +3.3\% $ln(\omega_c)$                                            & 0.02237 &  0.1240   & 0.6597 & 2.0205  & 0.9649 & 0.0      &   2.0328 & 1      &  6.4420 & -1.0   & 0.0    & 0.808270 & 0.811574  \\
\code{cosm103}    & Baseline -3.3\% $ln(\omega_c)$                                         & 0.02237 &  0.1161   & 0.6877 & 2.1541  & 0.9649 & 0.0      &   2.0328 & 1      &  6.4420 & -1.0   & 0.0    & 0.808075 & 0.811582  \\
\code{cosm104}    & Baseline +0.01 $n_s$                                                   & 0.02237 &  0.1200   & 0.6736 & 2.0684  & 0.9749 & 0.0      &   2.0328 & 1      &  6.4420 & -1.0   & 0.0    & 0.808166 & 0.811572  \\
\code{cosm105}    & Baseline -0.01 $n_s$                                                   & 0.02237 &  0.1200   & 0.6736 & 2.0999  & 0.9549 & 0.0      &   2.0328 & 1      &  6.4420 & -1.0   & 0.0    & 0.808177 & 0.811580  \\
\code{cosm106}    & Baseline +0.02 $n_{textrm{run }}$                                                 & 0.02237 &  0.1200   & 0.6736 & 2.0638  & 0.9649 & 0.02     &   2.0328 & 1      &  6.4420 & -1.0   & 0.0    & 0.808181 & 0.811586  \\
\code{cosm107}    & Baseline -0.02 $n_{textrm{run }}$                                                    & 0.02237 &  0.1200   & 0.6736 & 2.1045  & 0.9649 & -0.02    &   2.0328 & 1      &  6.4420 & -1.0   & 0.0    & 0.808168 & 0.811571  \\
\code{cosm108}    & Baseline +0.1 $w_0$                                                     & 0.02237 &  0.1200   & 0.6444 & 2.2390  & 0.9649 & 0.0      &   2.0328 & 1      &  6.4420 & -0.9   & 0.0    & 0.808177 & 0.811570  \\
\code{cosm109}    & Baseline -0.1 $w_0$                                                     & 0.02237 &  0.1200   & 0.7037 & 1.9465  & 0.9649 & 0.0      &   2.0328 & 1      &  6.4420 & -1.1   & 0.0    & 0.808161 & 0.811576  \\
\code{cosm110}    & Baseline +0.4 $w_a$, -0.1 $w_0$                                            & 0.02237 &  0.1200   & 0.6698 & 2.1219  & 0.9649 & 0.0      &   2.0328 & 1      &  6.4420 & -1.1   & 0.4    & 0.808170 & 0.811572  \\
\code{cosm111}    & Baseline -0.4 $w_a$, +0.1 $w_0$                                            & 0.02237 &  0.1200   & 0.6752 & 2.0639  & 0.9649 & 0.0      &   2.0328 & 1      &  6.4420 & -0.9   & -0.4   & 0.808179 & 0.811584  \\
\code{cosm112}    & Baseline +2\% $\sigma_8$                                                    & 0.02237 &  0.1200   & 0.6736 & 2.1672   & 0.9649 & 0.0      &   2.0328 & 1      &  6.4420 & -1.0   & 0.0    & 0.824120 & 0.827591  \\
\code{cosm113}    & Baseline -2\% $\sigma_8$                                                    & 0.02237 &  0.1200   & 0.6736 & 2.0021   & 0.9649 & 0.0      &   2.0328 & 1      &  6.4420 & -1.0   & 0.0    & 0.792107 & 0.795443  \\
\code{cosm114}    & Baseline +0.3 $nnu$?????, +3.3\% $ln(\omega_{c})$, +0.01 $n_s$                      & 0.02237 &  0.1240   & 0.6947 & 2.0463  & 0.9749 & 0.0      &   2.3328 & 1      &  6.4420 & -1.0   & 0.0    & 0.808245 & 0.811563  \\
\code{cosm115}    & Baseline -0.3 $nnu$?????, -3.3\% $ln(\omega_{c})$, -0.01 $n_s$                      & 0.02237 &  0.1161   & 0.6517 & 2.1211  & 0.9549 & 0.0      &   1.7328 & 1      &  6.4420 & -1.0   & 0.0    & 0.808089 & 0.811582  \\
\code{cosm116}    & Emulator grid around baseline cosmology                              & 0.02237 &  0.1200   & 0.6736 & 2.3938  & 0.9649 & 0.000    &  2.0328 & 1      &  6.4420 & -1.000 & 0.000  & 0.866133 & 0.869782  \\
\code{cosm117}    & Baseline +0.83\% $\ln(\omega_c)$                                         & 0.02237 &  0.1210   & 0.6701 & 2.0675e-09& 0.9649 & 0.0     & 2.0328 & 1      & 0.00064420 & -1.0   & 0.0    & 0.808205 & 0.811584  \\
\code{cosm118}    & Baseline -0.83\% $\ln(\omega_c)$                                         & 0.02237 &  0.1190   & 0.6771 & 2.1014e-09& 0.9649 & 0.0     & 2.0328 & 1      & 0.00064420 & -1.0   & 0.0    & 0.808152 & 0.811582  \\
\code{cosm119}    & Baseline +0.003 $n_s$                                                 & 0.02237 &  0.1200   & 0.6736 & 2.0794e-09& 0.9679 & 0.0     & 2.0328 & 1      & 0.00064420 & -1.0   & 0.0    & 0.808168 & 0.811573  \\
\code{cosm120}    & Baseline -0.003 $n_s$                                                 & 0.02237 &  0.1200   & 0.6736 & 2.0889e-09& 0.9619 & 0.0     & 2.0328 & 1      & 0.00064420 & -1.0   & 0.0    & 0.808181 & 0.811585  \\
\code{cosm121}    & Baseline +0.025 $w_0$                                                  & 0.02237 &  0.1200   & 0.6662 & 2.1211e-09& 0.9649 & 0.0     & 2.0328 & 1      & 0.00064420 & -0.975 & 0.0  & 0.808169 & 0.811571  \\
\code{cosm122}    & Baseline -0.025 $w_0$                                                  & 0.02237 &  0.1200   & 0.6810 & 2.0483e-09& 0.9649 & 0.0     & 2.0328 & 1      & 0.00064420 & -1.025 & 0.0  & 0.808170 & 0.811577  \\
\code{cosm123}    & Baseline +0.1 $w_a$, -0.025 $w_0$                                         & 0.02237 &  0.1200   & 0.6729 & 2.0915e-09& 0.9649 & 0.0     & 2.0328 & 1      & 0.00064420 & -1.025 & 0.1  & 0.808176 & 0.811580  \\
\code{cosm124}    & Baseline -0.1 $w_a$, +0.025 $w_0$                                         & 0.02237 &  0.1200   & 0.6742 & 2.0778e-09& 0.9649 & 0.0     & 2.0328 & 1      & 0.00064420 & -0.975 & -0.1 & 0.808175 & 0.811580  \\
\code{cosm125}    & Baseline +0.5\% $\sigma_8$                                               & 0.02237 &  0.1200   & 0.6736 & 2.1039e-09& 0.9649 & 0.0     & 2.0328 & 1      & 0.00064420 & -1.0   & 0.0    & 0.811995 & 0.815415  \\
\code{cosm126}    & Baseline -0.5\% $\sigma_8$                                               & 0.02237 &  0.1200   & 0.6736 & 2.0622e-09& 0.9649 & 0.0     & 2.0328 & 1      & 0.00064420 & -1.0   & 0.0    & 0.803908 & 0.807294  \\
\code{cosm130}    & Emulator grid around baseline cosmology                              & 0.02237 &  0.1200   & 0.6736 & 1.6140  & 0.9649 & 0.000    &  2.0328 & 1      &  6.4420 & -1.000 & 0.000  & 0.711201 & 0.714197  \\
\code{cosm131}    & Emulator grid around baseline cosmology                              & 0.02237 &  0.1086   & 0.7165 & 2.3146  & 0.9649 & 0.000    &  2.0328 & 1      &  6.4420 & -1.000 & 0.000  & 0.807866 & 0.811587  \\
\code{cosm132}    & Emulator grid around baseline cosmology                              & 0.02237 &  0.1200   & 0.6736 & 2.1791  & 0.9049 & 0.000    &  2.0328 & 1      &  6.4420 & -1.000 & 0.000  & 0.808189 & 0.811584  \\
\code{cosm133}    & Emulator grid around baseline cosmology                              & 0.02237 &  0.1200   & 0.6736 & 2.6144  & 0.9649 & 0.000    &  2.0328 & 1      &  6.4420 & -1.000 & 0.000  & 0.905163 & 0.908976  \\
\code{cosm134}    & Emulator grid around baseline cosmology                              & 0.02237 &  0.1326   & 0.6319 & 1.9066  & 0.9649 & 0.000    &  2.0328 & 1      &  6.4420 & -1.000 & 0.000  & 0.808458 & 0.811566  \\
\code{cosm135}    & Emulator grid around baseline cosmology                              & 0.02237 &  0.1200   & 0.6736 & 1.9904  & 1.0249 & 0.000    &  2.0328 & 1      &  6.4420 & -1.000 & 0.000  & 0.808160 & 0.811573  \\
\code{cosm136}    & Emulator grid around baseline cosmology                              & 0.02073 &  0.1192   & 0.6618 & 2.5239  & 0.9303 & 0.000    &  2.0328 & 1      &  6.4420 & -1.000 & 0.000  & 0.882475 & 0.886249  \\
\code{cosm137}    & Emulator grid around baseline cosmology                              & 0.02212 &  0.1271   & 0.6472 & 1.6540  & 0.9252 & 0.000    &  2.0328 & 1      &  6.4420 & -1.000 & 0.000  & 0.729693 & 0.732609  \\
\code{cosm138}    & Emulator grid around baseline cosmology                              & 0.02108 &  0.1138   & 0.6847 & 2.2282  & 0.9723 & 0.000    &  2.0328 & 1      &  6.4420 & -1.000 & 0.000  & 0.821432 & 0.825095  \\
\code{cosm139}    & Emulator grid around baseline cosmology                              & 0.02416 &  0.1128   & 0.7164 & 2.1681  & 0.9732 & 0.000    &  2.0328 & 1      &  6.4420 & -1.000 & 0.000  & 0.793003 & 0.796493  \\
\code{cosm140}    & Emulator grid around baseline cosmology                              & 0.02096 &  0.1221   & 0.6536 & 1.8126  & 0.9893 & 0.000    &  2.0328 & 1      &  6.4420 & -1.000 & 0.000  & 0.772033 & 0.775267  \\
\code{cosm141}    & Emulator grid around baseline cosmology                              & 0.02381 &  0.1272   & 0.6623 & 1.9945  & 0.9384 & 0.000    &  2.0328 & 1      &  6.4420 & -1.000 & 0.000  & 0.799575 & 0.802737  \\
\code{cosm142}    & Emulator grid around baseline cosmology                              & 0.02287 &  0.1130   & 0.7038 & 1.6701  & 0.9927 & 0.000    &  2.0328 & 1      &  6.4420 & -1.000 & 0.000  & 0.707082 & 0.710219  \\
\code{cosm143}    & Emulator grid around baseline cosmology                              & 0.02206 &  0.1278   & 0.6443 & 2.1084  & 0.9952 & 0.000    &  2.0328 & 1      &  6.4420 & -1.000 & 0.000  & 0.847522 & 0.850903  \\
\code{cosm144}    & Emulator grid around baseline cosmology                              & 0.02210 &  0.1130   & 0.6968 & 2.7653  & 0.9279 & 0.000    &  2.0328 & 1      &  6.4420 & -1.000 & 0.000  & 0.891360 & 0.895324  \\
\code{cosm145}    & Emulator grid around baseline cosmology                              & 0.02428 &  0.1186   & 0.6961 & 2.1634  & 0.9347 & 0.000    &  2.0328 & 1      &  6.4420 & -1.000 & 0.000  & 0.801404 & 0.804769  \\
\code{cosm146}    & Emulator grid around baseline cosmology                              & 0.02097 &  0.1180   & 0.6682 & 1.9020  & 0.9351 & 0.000    &  2.0328 & 1      &  6.4420 & -1.000 & 0.000  & 0.762696 & 0.765984 \\
\code{cosm147}    & Emulator grid around baseline cosmology                              & 0.02113 &  0.1215   & 0.6498 & 1.9081  & 0.9587 & 0.000    &  2.0328 & 1      &  6.4420 & -0.809 & -0.628  & 0.777157 & 0.780416  \\
\code{cosm148}    & Emulator grid around baseline cosmology                              & 0.02289 &  0.1201   & 0.6199 & 1.9629  & 0.9380 & 0.000    &  2.0328 & 1      &  6.4420 & -0.925 & 0.393  & 0.714913 & 0.717888  \\
\code{cosm149}    & Emulator grid around baseline cosmology                              & 0.02188 &  0.1200   & 0.6688 & 2.1521  & 0.9913 & 0.000    &  2.0328 & 1      &  6.4420 & -1.174 & 0.613  & 0.824854 & 0.828343  \\
\code{cosm150}    & Emulator grid around baseline cosmology                              & 0.02248 &  0.1216   & 0.7224 & 2.5099  & 0.9355 & 0.000    &  2.0328 & 1      &  6.4420 & -1.090 & -0.373  & 0.937655 & 0.941570  \\
\code{cosm151}    & Emulator grid around baseline cosmology                              & 0.02315 &  0.1254   & 0.6582 & 2.2686  & 0.9757 & 0.000    &  2.0328 & 1      &  6.4420 & -0.826 & -0.615  & 0.860820 & 0.864288  \\
\code{cosm152}    & Emulator grid around baseline cosmology                              & 0.02165 &  0.1148   & 0.6204 & 1.7965  & 0.9541 & 0.000    &  2.0328 & 1      &  6.4420 & -0.732 & -0.187  & 0.677885 & 0.680849  \\
\code{cosm153}    & Emulator grid around baseline cosmology                              & 0.02192 &  0.1199   & 0.6092 & 2.2946  & 0.9917 & 0.000    &  2.0328 & 1      &  6.4420 & -0.735 & -0.172  & 0.794389 & 0.797729  \\
\code{cosm154}    & Emulator grid around baseline cosmology                              & 0.02158 &  0.1148   & 0.7426 & 2.0689  & 0.9538 & 0.000    &  2.0328 & 1      &  6.4420 & -1.076 & -0.395  & 0.838698 & 0.842413  \\
\code{cosm155}    & Emulator grid around baseline cosmology                              & 0.02369 &  0.1184   & 0.6247 & 2.0723  & 0.9713 & 0.000    &  2.0328 & 1      &  6.4420 & -0.727 & -0.184  & 0.735302 & 0.738388  \\
\code{cosm156}    & Emulator grid around baseline cosmology                              & 0.02202 &  0.1261   & 0.6499 & 1.9738  & 0.9678 & 0.000    &  2.0328 & 1      &  6.4420 & -1.176 & 0.621  & 0.801974 & 0.805210  \\
\code{cosm157}    & Emulator grid around baseline cosmology                              & 0.02247 &  0.1214   & 0.6668 & 2.5108  & 0.9356 & 0.000    &  2.0328 & 1      &  6.4420 & -1.167 & 0.616  & 0.872315 & 0.875941  \\
\code{cosm158}    & Emulator grid around baseline cosmology                              & 0.02201 &  0.1262   & 0.6958 & 1.8626  & 0.9667 & 0.000    &  2.0328 & 1      &  6.4420 & -1.082 & -0.392  & 0.829816 & 0.833179  \\
\code{cosm159}    & Emulator grid around baseline cosmology                              & 0.02206 &  0.1261   & 0.5967 & 1.7977  & 0.9673 & 0.000    &  2.0328 & 1      &  6.4420 & -0.726 & -0.220  & 0.718521 & 0.721402  \\
\code{cosm160}    & Emulator grid around baseline cosmology                              & 0.02223 &  0.1185   & 0.7456 & 2.0963  & 0.9942 & 0.000    &  2.0328 & 1      &  6.4420 & -1.271 & 0.217  & 0.876756 & 0.880523  \\
\code{cosm161}    & Emulator grid around baseline cosmology                              & 0.02282 &  0.1274   & 0.7330 & 1.9688  & 0.9649 & 0.026    &  2.7283 & 1      &  6.4420 & -1.000 & 0.000  & 0.793066 & 0.796247  \\
\code{cosm162}    & Emulator grid around baseline cosmology                              & 0.02136 &  0.1048   & 0.6383 & 2.1592  & 0.9297 & -0.026   &   1.3521 & 1      &  6.4420 & -1.000 & 0.000  & 0.779589 & 0.783285  \\
\code{cosm163}    & Emulator grid around baseline cosmology                              & 0.02135 &  0.1290   & 0.7280 & 2.1689  & 0.9922 & -0.018   &   2.8575 & 1      &  6.4420 & -1.000 & 0.000  & 0.838824 & 0.842187  \\
\code{cosm164}    & Emulator grid around baseline cosmology                              & 0.02173 &  0.1091   & 0.6042 & 2.0003  & 0.9211 & 0.016    &  1.1769 & 1      &  6.4420 & -1.000 & 0.000  & 0.774159 & 0.777681  \\
\code{cosm165}    & Emulator grid around baseline cosmology                              & 0.02225 &  0.1278   & 0.7293 & 2.0676  & 1.0241 & 0.026    &  2.7558 & 1      &  6.4420 & -1.000 & 0.000  & 0.835954 & 0.839319  \\
\code{cosm166}    & Emulator grid around baseline cosmology                              & 0.02306 &  0.1151   & 0.6826 & 2.2779  & 0.9691 & 0.038    &  1.9089 & 1      &  6.4420 & -1.000 & 0.000  & 0.837463 & 0.841106  \\
\code{cosm167}    & Emulator grid around baseline cosmology                              & 0.02248 &  0.1400   & 0.7050 & 1.7321  & 0.9715 & -0.017   &   2.8889 & 1      &  6.4420 & -1.000 & 0.000  & 0.768419 & 0.771255  \\
\code{cosm168}    & Emulator grid around baseline cosmology                              & 0.02157 &  0.1084   & 0.6070 & 2.5378  & 0.9275 & 0.016    &  1.1911 & 1      &  6.4420 & -1.000 & 0.000  & 0.871407 & 0.875401  \\
\code{cosm169}    & Emulator grid around baseline cosmology                              & 0.02189 &  0.1222   & 0.6474 & 1.8067  & 0.9898 & 0.038    &  1.9109 & 1      &  6.4420 & -1.000 & 0.000  & 0.777925 & 0.781158  \\
\code{cosm170}    & Emulator grid around baseline cosmology                              & 0.02319 &  0.1076   & 0.6418 & 1.7994  & 0.9387 & -0.026   &   1.3411 & 1      &  6.4420 & -1.000 & 0.000  & 0.716059 & 0.719332  \\
\code{cosm171}    & Emulator grid around baseline cosmology                              & 0.02348 &  0.1272   & 0.6733 & 2.2585  & 0.9762 & -0.038   &   2.1543 & 1      &  6.4420 & -1.000 & 0.000  & 0.852878 & 0.856267  \\
\code{cosm172}    & Emulator grid around baseline cosmology                              & 0.02282 &  0.1032   & 0.6369 & 2.1259  & 0.9012 & 0.017    &  1.1954 & 1      &  6.4420 & -1.000 & 0.000  & 0.765650 & 0.769278  \\
\code{cosm173}    & Emulator grid around baseline cosmology                              & 0.02322 &  0.1161   & 0.6800 & 1.8904  & 0.9628 & 0.038    &  1.9049 & 1      &  6.4420 & -1.000 & 0.000  & 0.763962 & 0.767255  \\
\code{cosm174}    & Emulator grid around baseline cosmology                              & 0.02302 &  0.1064   & 0.6427 & 2.4889  & 0.9437 & -0.026   &   1.3242 & 1      &  6.4420 & -1.000 & 0.000  & 0.840113 & 0.843996  \\
\code{cosm175}    & Emulator grid around baseline cosmology                              & 0.02173 &  0.1336   & 0.6432 & 1.7429  & 0.9898 & -0.003   &   2.7456 & 1      &  6.4420 & -0.911 & 0.350  & 0.708760 & 0.711484 \\
\code{cosm176}    & Emulator grid around baseline cosmology                              & 0.02238 &  0.1199   & 0.6972 & 2.3120  & 0.9459 & 0.036    &  1.9043 & 1      &  6.4420 & -1.222 & 0.339  & 0.892483 & 0.896318  \\
\code{cosm177}    & Emulator grid around baseline cosmology                              & 0.02239 &  0.1344   & 0.6820 & 2.0641  & 1.0002 & 0.007    &  2.8643 & 1      &  6.4420 & -0.757 & -0.443  & 0.806026 & 0.809110  \\
\code{cosm178}    & Emulator grid around baseline cosmology                              & 0.02234 &  0.1204   & 0.6542 & 1.9665  & 0.9424 & 0.037    &  1.8987 & 1      &  6.4420 & -0.874 & -0.455  & 0.791239 & 0.794555  \\
\code{cosm179}    & Emulator grid around baseline cosmology                              & 0.02240 &  0.1067   & 0.5881 & 2.2365  & 0.9308 & -0.003   &   1.1884 & 1      &  6.4420 & -0.755 & -0.435  & 0.775969 & 0.779541  \\
\code{cosm180}    & Emulator grid around baseline cosmology                              & 0.02258 &  0.1209   & 0.7451 & 2.2790  & 0.9796 & -0.034   &   2.1722 & 1      &  6.4420 & -1.108 & -0.274  & 0.894071 & 0.897833  \\
\code{cosm181}    & Emulator grid around baseline cosmology                              & 0.02169 &  0.1112   & 0.5745 & 2.0651  & 0.9336 & -0.013   &   1.4059 & 1      &  6.4420 & -0.910 & 0.350  & 0.730036 & 0.733292   \\
    

\end{longtable}
\end{landscape}

==> outline_to_do.tex <==
\section{Outline and To-Do List}
\TODO{Remove this outline later!}

\subsection{Outline}
\begin{enumerate}
    \item Introduction: introduce/motivate LSS, N-body, \Abacus, \AbacusSummit
    
    \item \AbacusSummit{} Simulation Details
    \begin{enumerate}
        \item Initial conditions: generated with zeldovich-PLT, rescaled to z=5, z init = 99, briefly mention performance on Rhea, CAMB power spectrum. Mention unique PID. 
        \item Code Parameters: Make a table following AbacusCosmos paper of choices for: timestepping, force softening scheme, IC LPT/etc, proper softening, softening length.
        \item Data Products: 
            \begin{enumerate}
                \item Full particle snapshots (RV, PID)
                \item Subsamples, separated into field/halo/3/7
                \item Halo catalogues and merger tree PIDs
                \item Lightcones and density maps
            \end{enumerate}
       \item Cosmologies: include corner plot, perhaps a full table (or not). \item Simulations: include full table? or condensed description of boxes with link to e-table. 
    \end{enumerate}
    
     \item \Abacus{}
    \begin{enumerate}
        \item Force Solver Algorithm and Serial Method: far field, near field, slab pipeline  
        \item Massive parallelization: convolution parallelization, singlestep parallelization, manifests, resulting  constraints
        \item Halo finder: brief algorithm  description, brief paragraph about validation, mainly direct readers to Boryana's paper
        \item Light cones: brief description of module/interpolation, direct readers to code paper
        \item Force softening scheme; proper softening 
        \item Time stepping criteria / global timestepping 
        \item Data processing: extensive checksumming; lots of compression (multiple layers, describe each briefly) 
    \end{enumerate}
    
    \item Suite Performance 
        \begin{enumerate}
            \item Mention production performed with assembly line, briefly describe but don't belabor. 
            \item describe performance tricks: VSX instrincs, SMT, thread pools, NUMA locality, GPU threads, etc 
            \item singlestep performance: break it down by dependency; GPU performance 
            \item convolution performance
            \item consider including strong/weak scaling tables
        \end{enumerate}
    \item Validation 
        \begin{enumerate}
            \item Mass resolution convergence tests (HMF, one line for each of \AbacusSummit resolutions)
            \item Linear theory test
            \item Consider comparing \AbacusSummit (HMF? Power spectrum?) to Aemulus or CosmicEMU 
            \item Show timestepping convergence with $2660^3$ boxes
        \end{enumerate}
    \item Conclusion: sum up \AbacusSummit, where it's available. 
    \item Acknowledgements
\end{enumerate}

\subsection{TO-DO}
\begin{itemize}
\item Halo Finder:
\begin{itemize}
    \item plot: halo profiles vs timestep
    \item plot: halo profiles vs softening
    \item plot: comparisons against Rockstar
    \item plot: comparing HMF against published HMF (see Aemulus) over a range of redshifts
\end{itemize}
\item Lightcones:
\begin{itemize}
    \item \st{describe choices of interpolation of particles crossing the light cone}
    \item \st{describe that transverse boundaries are not safe to use}
\end{itemize} 

\item Validation:
\begin{itemize}
    \item include plot: of linear theory tests
    \item plot: mass resolution convergence tests (HMF w/ three lines, one for each resolution in AbacusSummit) 
    \item plot: matter power spectrum comparison to known cosmic emulators (e.g. CosmicEmu) at variety of redshifts.
    \item plot: halo power spectrum comparison to Aemulus at variety of redshifts.
    \item plot/describe: timestepping convergence.
    \item dig up Lehman’s old email about this and look for existing 2660 boxes. time stepping convergence tests can	be done with correct particle mass resolution, doesn’t need to be same Np.
    \item \st{descope: scale-free figure and results} 
\end{itemize} 

\item Performance:
\begin{itemize}
    \item fix: unaccounted time (Lehman thinks it might be related to MPI calls in a precondition) 
    \item \st{create: weak scaling table, early times with Poisson ICs}
    \item \st{create: strong scaling test at $7000^3$ scale, take it up to 80 nodes, watch for GPU overheads}
    \item create: table mimicking Euclid paper of breakdowns where we spend time in Abacus
    \item \st{quote: SMT 1/2/4 performances}
    \item \st{discuss: NUMA locality, different thread pools (IO, GPU, openMP)}
    \item plot: performance over steps (w/ lines of GPU, CPU, and convolution, or perhaps a more detailed breakdown) 
    \item plot/discuss: node to node variation, including spinning 
    \item request: Lehman’s paragraph about VSX kernels 
    \item plot: GPU directs rate vs directs per particle
    \item run: nvidia profiler to figure out exactly how many ops are in our kernel 
    \item plot: fraction of theoretical peak performance
    \item discuss: IC performance on rhea 
    \item discuss: post processing performance on rhea 
\end{itemize}

\item{Data Products:} 
\begin{itemize}
    \item describe: all our various compression schemes. float to RVint (lossy compression, mention precision) to blosc (lossless to ASDF)
    \item \st{describe: assembly line structure}
    \item \st{describe: dynamic disBatch scheduling that absorbs heterogeneous workload in post-processing}
    \item  \st{discuss: we have checksums everywhere! We do on the fly checksums inside abacus before data ever hits disks, then every time we read in the data during post-processing pipeline, it’s automatically checksummed and verified. we also checksum the compressed data products and transfer them to final destination.} 

    \item \st{belabor: importance of our density estimates in the PIDs. That’s a lot of particles at a lot of z’s with densities!}
    \item request: Lehman’s paragraph about ASDF compression scene and file format. 
    \item \st{describe: healpix maps $N_{side}$ choice to serve weak lensing}
\end{itemize}

\item Visualizations:
\begin{itemize}
    \item think about: 2-3 full-page figures to include e.g. Bo’s light cones, but so they fit on a page? Abacus timeslice? 
\end{itemize}

\end{itemize}
